Software Engineering and Foundation Models: Insights from Industry Blogs Using a Jury of Foundation Models

Foundation models (FMs) such as large language models (LLMs) have significantly impacted many fields, including software engineering (SE). The interaction between SE and FMs has led to the integration of FMs into SE practices (FM4SE) and the application of SE methodologies to FMs (SE4FM). While several literature surveys exist on academic contributions to these trends, we are the first to provide a practitioner's view. We analyze 155 FM4SE and 997 SE4FM blog posts from leading technology companies, leveraging an FM-powered surveying approach to systematically label and summarize the discussed activities and tasks. We observed that while code generation is the most prominent FM4SE task, FMs are leveraged for many other SE activities such as code understanding, summarization, and API recommendation. The majority of blog posts on SE4FM are about model deployment & operation, and system architecture & orchestration. Although the emphasis is on cloud deployments, there is a growing interest in compressing FMs and deploying them on smaller devices such as edge or mobile devices. We outline eight future research directions inspired by our gained insights, aiming to bridge the gap between academic findings and real-world applications. Our study not only enriches the body of knowledge on practical applications of FM4SE and SE4FM but also demonstrates the utility of FMs as a powerful and efficient approach in conducting literature surveys within technical and grey literature domains. Our dataset, results, code and used prompts can be found in our online replication package at https://github.com/SAILResearch/fmse-blogs.

==> sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}

==> sections/rq3.tex <==
\subsection{RQ3: \rqthree}\label{sec:rq3}

\motivation

\approach

\findings

customize, optimize, then deploy: https://developer.nvidia.com/blog/streamline-ai-powered-app-development-with-nvidia-rtx-ai-toolkit-for-windows-rtx-pcs/

template support:
https://devblogs.microsoft.com/semantic-kernel/enhanced-templating-in-semantic-kernel-for-python/

guardrails:
https://aws.amazon.com/blogs/machine-learning/build-safe-and-responsible-generative-ai-applications-with-guardrails/

Model access:
https://aws.amazon.com/blogs/dotnet/getting-started-with-amazon-bedrock-in-net-applications/

% \begin{figure*}[h]
% \centering
% \includegraphics[width=\textwidth]{figs/se4fm_challenge_per_company}
% \caption{SE for FM challenges faced by companies.}
% \label{fig:se4fm_challenge_per_company}
% \end{figure*}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figs/se4fm_Challenge_Label_percentage}
% \caption{Challenges faced in SE for FM.}
% \label{fig:se4fm_Challenge_Label_percentage}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figs/se4fm_Methodology_Label_percentage}
% \caption{Methodologies used in SE for FM.}
% \label{fig:se4fm_Methodology_Label_percentage}
% \end{figure}

% \begin{figure*}[h]
% \centering
% \includegraphics[width=\textwidth]{figs/se4fm_methodology_vs_challenge}
% \caption{SE for FM Methodologies and Challenges.}
% \label{fig:se4fm_methodology_vs_challenge}
% \end{figure*}

% \begin{figure*}[h]
% \centering
% \includegraphics[width=\textwidth]{figs/se4fm_challenge_vs_methodology}
% \caption{SE for FM challenges and methodologies.}
% \label{fig:se4fm_challenge_vs_methodology}
% \end{figure*}


% claude-3-haiku@20240307,gemini-1.5-flash-002,0.5796019900497513
% claude-3-haiku@20240307,gpt-4o-mini-2024-07-18,0.5202952029520296
% claude-3-haiku@20240307,human,0.5672436750998668
% claude-3-haiku@20240307,voted_three,0.708955223880597
% gemini-1.5-flash-002,gpt-4o-mini-2024-07-18,0.7011278195488722
% gemini-1.5-flash-002,human,0.7893258426966292
% gemini-1.5-flash-002,voted_three,0.8668373879641486
% gpt-4o-mini-2024-07-18,human,0.8202731847591661
% gpt-4o-mini-2024-07-18,voted_three,0.7983193277310925
% human,voted_three,0.7893258426966292


\begin{table*}[t]
\centering
\caption{Cohen's Kappa agreement between annotators for labelling categories (SE4FM vs. FM4SE vs. unrelated) among 50 Samples.}
\label{tab:my-table}
\begin{tabular}{lrrrrrr}
\toprule
Model                      & c35-sonnet & c3-haiku & g1.5-flash & g1.5-pro & gpt4o-mini & human         \\ \midrule
claude-3-5-sonnet@20240620 & --                         & 0.38                    & \textbf{0.64}        & \textbf{0.75}      & 0.58                   & \textbf{0.70} \\
claude-3-haiku@20240307    & 0.38                       & --                      & 0.56                 & 0.36               & 0.50                   & 0.57          \\
gemini-1.5-flash-002       & \textbf{0.64}              & 0.56                    & --                   & 0.61               & \textbf{0.68}          & \textbf{0.79} \\
gemini-1.5-pro-002         & \textbf{0.75}              & 0.36                    & 0.61                 & --                 & \textbf{0.63}                   & \textbf{0.74} \\
gpt-4o-mini-2024-07-18     & 0.58                       & 0.50                    & \textbf{0.68}        & \textbf{0.63}      & --                     & \textbf{0.82} \\
human                      & \textbf{0.70}              & 0.57                    & \textbf{0.79}        & \textbf{0.74}      & \textbf{0.82}          & --            \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Cohen's Kappa agreement between annotators for labelling categories (SE4FM vs. FM4SE vs. unrelated) among 50 Samples.}
\label{tab:my-table}
\begin{tabular}{lrrrrrrrr}
\toprule
Model                      & c35-sonnet & c3-haiku & g1.5-flash & g1.5-pro & gpt4o-mini & human & voted\_all & voted\_three \\ \midrule
claude-3-5-sonnet@20240620 & --         & 0.38     & 0.64       & 0.75     & 0.58       & 0.70  & 0.77       & 0.77         \\
claude-3-haiku@20240307    & 0.38       & --       & 0.56       & 0.36     & 0.50       & 0.57  & 0.57       & 0.57         \\
gemini-1.5-flash-002       & 0.64       & 0.56     & --         & 0.61     & 0.68       & 0.79  & 0.86       & 0.86         \\
gemini-1.5-pro-002         & 0.75       & 0.36     & 0.61       & --       & 0.63       & 0.74  & 0.73       & 0.73         \\
gpt-4o-mini-2024-07-18     & 0.58       & 0.50     & 0.68       & 0.63     & --         & 0.82  & 0.82       & 0.82         \\
human                      & 0.70       & 0.57     & 0.79       & 0.74     & 0.82       & --    & \textbf{0.93}       & \textbf{0.93}         \\
voted\_all                 & 0.77       & 0.57     & 0.86       & 0.73     & 0.82       & \textbf{0.93}  & --         & \textbf{1.00}         \\
voted\_three               & 0.77       & 0.57     & 0.86       & 0.73     & 0.82       & \textbf{0.93}  & \textbf{1.00}       & --           \\ \bottomrule
\end{tabular}
\end{table*}


\begin{table}[t]
\centering
\caption{Cohen's Kappa agreement between annotators for labelling categories (SE4FM vs. FM4SE vs. unrelated) among 698 Samples.}
\label{tab:my-table}
\begin{tabular}{lrrr}
\toprule
Model                   & c3-haiku & g1.5-flash & gpt4o-mini \\ \midrule
claude-3-haiku@20240307 & --                      & 0.47                 & 0.46                   \\
gemini-1.5-flash-002    & 0.47                    & --                   & \textbf{0.68}          \\
gpt-4o-mini-2024-07-18  & 0.46                    & \textbf{0.68}        & --                     \\ \bottomrule
\end{tabular}
\end{table}


\begin{table*}[t]
\caption{Cohen's Kappa Agreement Between LLMs for Labelling Based on Any (Partial) Label Match.}
\centering
\label{tab:my-table}
\begin{tabular}{l|rrrrr|rrrrr|rrrrr}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{5}{c|}{Category (e.g., SE4FM or FM4SE)}                                                                                  & \multicolumn{5}{c|}{Activity (e.g., Software development)}                                                                            & \multicolumn{5}{c}{Task (e.g., code generation)}                                                                                     \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l|}{human} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l|}{human} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l}{human} \\ \midrule
claude-3.5-sonnet     & --                         & 0.44                    & 0.48                    & 0.10                    & 0.28                       & --                         & 0.42                    & 0.45                    & 0.15                    & 0.42                       & --                         & 0.17                    & 0.33                    & 0.14                    & 0.43                      \\
gemini-1.5-flash      & 0.44                       & --                      & 0.59                    & 0.15                    & 0.06                       & 0.42                       & --                      & 0.53                    & 0.26                    & 0.14                       & 0.17                       & --                      & 0.25                    & 0.13                    & 0.12                      \\
gemini-1.5-pro        & 0.48                       & 0.59                    & --                      & 0.18                    & 0.15                       & 0.45                       & 0.53                    & --                      & 0.21                    & 0.27                       & 0.33                       & 0.25                    & --                      & 0.22                    & 0.25                      \\
gpt-4o-mini           & 0.10                       & 0.15                    & 0.18                    & --                      & 0.06                       & 0.15                       & 0.26                    & 0.21                    & --                      & 0.09                       & 0.14                       & 0.13                    & 0.22                    & --                      & 0.06                      \\
human (50 samples)    & 0.28                       & 0.06                    & 0.15                    & 0.06                    & --                         & 0.42                       & 0.14                    & 0.27                    & 0.09                    & --                         & 0.43                       & 0.12                    & 0.25                    & 0.06                    & --                        \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\caption{Cohen's Kappa Agreement Between LLMs for Labelling Based on Any (Partial) Label Match.}
\centering
\label{tab:my-table}
\begin{tabular}{l|rrrrr|rrrrr|rrrrr}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{5}{c|}{Category (e.g., SE4FM or FM4SE)}                                                                                  & \multicolumn{5}{c|}{Activity (e.g., Software development)}                                                                            & \multicolumn{5}{c}{Task (e.g., code generation)}                                                                                     \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l|}{human} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l|}{human} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l}{human} \\ \midrule
claude-3.5-sonnet     & --                         & 0.44                    & 0.48                    & 0.10                    & 0.28                       & --                         & 0.42                    & 0.45                    & 0.15                    & 0.42                       & --                         & 0.17                    & 0.33                    & 0.14                    & 0.43                      \\
gemini-1.5-flash      & 0.44                       & --                      & 0.59                    & 0.15                    & 0.06                       & 0.42                       & --                      & 0.53                    & 0.26                    & 0.14                       & 0.17                       & --                      & 0.25                    & 0.13                    & 0.12                      \\
gemini-1.5-pro        & 0.48                       & 0.59                    & --                      & 0.18                    & 0.15                       & 0.45                       & 0.53                    & --                      & 0.21                    & 0.27                       & 0.33                       & 0.25                    & --                      & 0.22                    & 0.25                      \\
gpt-4o-mini           & 0.10                       & 0.15                    & 0.18                    & --                      & 0.06                       & 0.15                       & 0.26                    & 0.21                    & --                      & 0.09                       & 0.14                       & 0.13                    & 0.22                    & --                      & 0.06                      \\
human (50 samples)    & 0.28                       & 0.06                    & 0.15                    & 0.06                    & --                         & 0.42                       & 0.14                    & 0.27                    & 0.09                    & --                         & 0.43                       & 0.12                    & 0.25                    & 0.06                    & --                        \\ \bottomrule
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\caption{Cohen's Kappa Agreement Between LLMs for Labelling Based on Exact Label Match.}
\centering
\label{tab:my-table}
\begin{tabular}{l|rrrrr|rrrrr|rrrrr}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{5}{c|}{Category (e.g., SE4FM or FM4SE)}                                                                                  & \multicolumn{5}{c|}{Activity (e.g., Software development)}                                                                            & \multicolumn{5}{c}{Task (e.g., code generation)}                                                                                     \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l|}{human} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l|}{human} & \multicolumn{1}{c}{claude} & \multicolumn{1}{c}{g-f} & \multicolumn{1}{c}{g-p} & \multicolumn{1}{c}{gpt} & \multicolumn{1}{l}{human} \\ \midrule
claude-3.5-sonnet     & --                         & 0.41                    & 0.44                    & 0.10                    & 0.26                       & --                         & 0.30                    & 0.22                    & 0.14                    & 0.37                       & --                         & 0.10                    & 0.13                    & 0.11                    & 0.39                      \\
gemini-1.5-flash      & 0.41                       & --                      & 0.53                    & 0.16                    & 0.05                       & 0.30                       & --                      & 0.21                    & 0.20                    & 0.07                       & 0.10                       & --                      & 0.10                    & 0.07                    & 0.08                      \\
gemini-1.5-pro        & 0.44                       & 0.53                    & --                      & 0.20                    & 0.10                       & 0.22                       & 0.21                    & --                      & 0.13                    & 0.11                       & 0.13                       & 0.10                    & --                      & 0.06                    & 0.05                      \\
gpt-4o-mini           & 0.10                       & 0.16                    & 0.20                    & --                      & 0.06                       & 0.14                       & 0.20                    & 0.13                    & --                      & 0.08                       & 0.11                       & 0.07                    & 0.06                    & --                      & 0.05                      \\
human (50 samples)    & 0.26                       & 0.05                    & 0.10                    & 0.06                    & --                         & 0.37                       & 0.07                    & 0.11                    & 0.08                    & --                         & 0.39                       & 0.08                    & 0.05                    & 0.05                    & --                        \\ \bottomrule
\end{tabular}
\end{table*}


==> tables/cohen_kappa_threshold.tex <==
\begin{table}[t]
\centering
\caption{Kappa Values and Strength of Agreement}
\label{tab:kappa_values}
\begin{tabular}{ll}
\toprule
Kappa Value & Strength of Agreement \\ \midrule
$<$ 0.45                        & Poor                  \\
0.45 -- 0.62                    & Moderate              \\
0.63 -- 0.78                    & Substantial           \\
$>$ 0.78                        & Excellent             \\ \bottomrule
\end{tabular}
\end{table}

==> tables/llm_jury_full_dataset.tex <==
\begin{table*}[t]
\centering
\caption{Cohen's Kappa between LLMs across the full dataset for SE-FM area, SE4FM activity, and FM4SE activity classification tasks.}
\label{tab:llm_jury_full_dataset}
\begin{tabular}{l|rrr|rrr|rrr}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{SE-FM Area (4,364 Blogs)}               & \multicolumn{3}{c|}{FM4SE Activity (160 Blogs)}           & \multicolumn{3}{c}{SE4FM Activity (1,078 Blogs)}            \\
                       & Gemini-1.5-F  & GPT-4o-m   & Qwen2         & Gemini-1.5-F  & GPT-4o-m   & Qwen2         & Gemini-1.5-F  & GPT-4o-m   & Qwen2         \\ \midrule
Gemini-1.5-Flash-002   & --            & 0.61          & 0.68          & --            & 0.73          & 0.69          & --            & 0.51          & 0.57          \\
GPT-4o-mini-2024-07-18 & 0.61          & --            & 0.76          & 0.73          & --            & 0.75          & 0.51          & --            & 0.50          \\
Qwen2-72B-Instruct     & 0.68          & 0.76          & --            & 0.69          & 0.75          & --            & 0.57          & 0.50          & --            \\ \midrule
\textbf{\ourmethod}        & \textbf{0.77} & \textbf{0.83} & \textbf{0.91} & \textbf{0.82} & \textbf{0.90} & \textbf{0.84} & \textbf{0.77} & \textbf{0.69} & \textbf{0.77} \\ \bottomrule
\end{tabular}
\end{table*}
